A Brown Theorem for Dehn functions of graphs of groups

We prove an upper bound on the Dehn function of a group $G$ acting cellularly, cocompactly, and without inversions on a simply connected CW complex $X$ in terms of the Dehn functions of the vertex stabilizers, the Dehn function of $X$, and the distortion of the edge stabilizers, provided that $X$ is either a tree or the stabilizer of each $2$-cell has finite index in the stabilizer of every edge in its boundary. This provides a Dehn function analogue of Brown's Theorem for finiteness properties and an answer to a question of Zaremsky in these cases. We also prove analogues of our result for higher Dehn functions when $X$ is a tree.

==> figures/base.tex <==
\RequirePackage{pgfkeys}
\pgfkeys{
    /baseimage/.is family, /baseimage,
    sidelength/.initial=4,
    circleradius/.initial=8mm,
    intervalthickness/.initial=7mm,
    outlinethickness/.initial=0.8pt,
    pathoffset/.initial={0.2*\intervalthickness},
    innerpathoffset/.initial={\pgfkeysvalueof{/baseimage/pathoffset}},
    outerpathoffset/.initial={\pgfkeysvalueof{/baseimage/pathoffset}},
    Ax/.initial={-0.5*\sidelength},
    Ay/.initial={-sqrt(3)/6*\sidelength},
    Az/.initial=0,
    Bx/.initial={0.5*\sidelength},
    By/.initial={-sqrt(3)/6*\sidelength},
    Bz/.initial=0,
    Cx/.initial={0},
    Cy/.initial={sqrt(3)/3*\sidelength},
    Cz/.initial=0,
}

\NewDocumentCommand{\baseImage}{O{}}{%
    \pgfkeys{/baseimage, #1}
    \def\sidelength{\pgfkeysvalueof{/baseimage/sidelength}}
    \def\circleradius{\pgfkeysvalueof{/baseimage/circleradius}}
    \def\intervalthickness{\pgfkeysvalueof{/baseimage/intervalthickness}}
    \def\outlinethickness{\pgfkeysvalueof{/baseimage/outlinethickness}}
    \def\pathoffset{\pgfkeysvalueof{/baseimage/pathoffset}}
    \def\innerpathoffset{\pgfkeysvalueof{/baseimage/innerpathoffset}}
    \def\outerpathoffset{\pgfkeysvalueof{/baseimage/outerpathoffset}}

    \def\baseimageAx{\pgfkeysvalueof{/baseimage/Ax}}
    \def\baseimageAy{\pgfkeysvalueof{/baseimage/Ay}}
    \def\baseimageAz{\pgfkeysvalueof{/baseimage/Az}}
    \def\baseimageBx{\pgfkeysvalueof{/baseimage/Bx}}
    \def\baseimageBy{\pgfkeysvalueof{/baseimage/By}}
    \def\baseimageBz{\pgfkeysvalueof{/baseimage/Bz}}
    \def\baseimageCx{\pgfkeysvalueof{/baseimage/Cx}}
    \def\baseimageCy{\pgfkeysvalueof{/baseimage/Cy}}
    \def\baseimageCz{\pgfkeysvalueof{/baseimage/Cz}}
    \def\baseimageAuto{auto}

    \coordinate (A) at ({\baseimageAx},{\baseimageAy},{\baseimageAz});
    \coordinate (B) at ({\baseimageBx},{\baseimageBy},{\baseimageBz});
    \coordinate (C) at ({\baseimageCx},{\baseimageCy},{\baseimageCz});
    \coordinate (Center) at (barycentric cs:A=1,B=1,C=1);

    \coordinate (ABCenter) at ($(A)!\circleradius!(B)$);
    \coordinate (ABInner)  at ($(ABCenter)!\innerpathoffset!($(ABCenter)+(C)-($(A)!(C)!(B)$)$)$);
    \coordinate (ABOuter)  at ($(ABCenter)!\outerpathoffset!180:($(ABCenter)+(C)-($(A)!(C)!(B)$)$)$);

    \coordinate (ACCenter) at ($(A)!\circleradius!(C)$);
    \coordinate (ACInner)  at ($(ACCenter)!\innerpathoffset!($(ACCenter)+(B)-($(A)!(B)!(C)$)$)$);
    \coordinate (ACOuter)  at ($(ACCenter)!\outerpathoffset!180:($(ACCenter)+(B)-($(A)!(B)!(C)$)$)$);

    \coordinate (BACenter) at ($(B)!\circleradius!(A)$);
    \coordinate (BAInner)  at ($(BACenter)!\innerpathoffset!($(BACenter)+(C)-($(B)!(C)!(A)$)$)$);
    \coordinate (BAOuter)  at ($(BACenter)!\outerpathoffset!180:($(BACenter)+(C)-($(B)!(C)!(A)$)$)$);

    \coordinate (BCCenter) at ($(B)!\circleradius!(C)$);
    \coordinate (BCInner)  at ($(BCCenter)!\innerpathoffset!($(BCCenter)+(A)-($(B)!(A)!(C)$)$)$);
    \coordinate (BCOuter)  at ($(BCCenter)!\outerpathoffset!180:($(BCCenter)+(A)-($(B)!(A)!(C)$)$)$);

    \coordinate (CACenter) at ($(C)!\circleradius!(A)$);
    \coordinate (CAInner)  at ($(CACenter)!\innerpathoffset!($(CACenter)+(B)-($(C)!(B)!(A)$)$)$);
    \coordinate (CAOuter)  at ($(CACenter)!\outerpathoffset!180:($(CACenter)+(B)-($(C)!(B)!(A)$)$)$);

    \coordinate (CBCenter) at ($(C)!\circleradius!(B)$);
    \coordinate (CBInner)  at ($(CBCenter)!\innerpathoffset!($(CBCenter)+(A)-($(C)!(A)!(B)$)$)$);
    \coordinate (CBOuter)  at ($(CBCenter)!\outerpathoffset!180:($(CBCenter)+(A)-($(C)!(A)!(B)$)$)$);

    \path[overlay,name path=ACircle] (A) circle[radius=\circleradius];
    \path[overlay,name path=BCircle] (B) circle[radius=\circleradius];
    \path[overlay,name path=CCircle] (C) circle[radius=\circleradius];

    \foreach \X in {A,B,C}{
            \foreach \Y in {A,B,C}{
                    \foreach \Side in {Inner,Outer}{
                            \if\X\Y\else
                                \path[overlay,name path=Ray\X\Y\Side]
                                (\X\Y\Side)
                                -- ($(\X\Y\Side)!100!(\Y\X\Side)$);
                            \fi
                        }
                }
        }

    % Backward-compatible aliases
    \coordinate (AStart)  at (ACOuter);
    \coordinate (AStartP) at (ACInner);
    \coordinate (AEnd)    at (CAOuter);
    \coordinate (AEndP)   at (CAInner);
    \coordinate (BStart)  at (CBOuter);
    \coordinate (BStartP) at (CBInner);
    \coordinate (BEnd)    at (BCOuter);
    \coordinate (BEndP)   at (BCInner);

    \coordinate (PathStartCenter) at ($(A)!0.2*\circleradius!(C)$);
    \coordinate (PathStart) at ($(PathStartCenter)!\pathoffset!180:($(PathStartCenter)+(B)-($(A)!(B)!(C)$)$)$);
    \coordinate (PathEndCenter) at ($(B)!0.2*\circleradius!(C)$);
    \coordinate (PathEnd)   at ($(PathEndCenter)!\pathoffset!180:($(PathEndCenter)+(A)-($(B)!(A)!(C)$)$)$);

    \tikzset{
        thick interval/.style={
                draw=black,
                fill=white,
                line width=\outlinethickness,
                line cap=round,
                line join=round,
                double=white,
                double distance=\intervalthickness
            },
        loop path/.style={
                thick,
                line cap=round,
                line join=round
            },
        connection path/.style={
                decorate,
                decoration={coil,aspect=0,segment length=5pt,amplitude=1pt}
            },
        every circle/.style={radius=1.5pt}
    }
}
\NewDocumentCommand{\ComputeCoordinates}{}{
    \coordinate (AMid) at ($1/2*(AStart)+1/2*(AEnd)$);
    \coordinate (AMidP) at ($1/2*(AStartP)+1/2*(AEndP)$);
    \coordinate (BMid) at ($1/2*(BStart)+1/2*(BEnd)$);
    \coordinate (BMidP) at ($1/2*(BStartP)+1/2*(BEndP)$);
    \coordinate (CMid) at ($1/2*(AStart)+1/2*(BEnd)$);
    \coordinate (CMidP) at ($1/2*(AStartP)+1/2*(BEndP)$);
}
